On Optimal Approximations for $k$-Submodular Maximization via Multilinear Extension

We investigate a more generalized form of submodular maximization, referred to as $k$-submodular maximization, with applications across social networks and machine learning domains. In this work, we propose the multilinear extension of $k$-submodular functions and unified Frank-Wolfe-type frameworks based on that. Our frameworks accomodate 1) monotone or non-monotone functions, and 2) various constraint types including matroid constraints, knapsack constraints, and their combinations. Notably, we attain an asymptotically optimal $1/2$-approximation for monotone $k$-submodular maximization problems with knapsack constraints, surpassing the previous $1/3$-approximation. The foundation for our analysis stems from new insights into specific linear and monotone properties pertaining to the multilinear extension.

==> todo.tex <==
%to do list 

%4.1-4.7 section 2 & section 3 & section 4
% writing and modification

%4.8-4.15 section 5 & section 6
% writing and modification

%4.15 - 4.28 
% introduction 
% technique overview 
% writing and modification


%5.1-5.4 
%5.4-5.7
%5.7-5.10
